Informed Down-Sampled Lexicase Selection: Identifying productive training cases for efficient problem solving

Genetic Programming (GP) often uses large training sets and requires all individuals to be evaluated on all training cases during selection. Random down-sampled lexicase selection evaluates individuals on only a random subset of the training cases allowing for more individuals to be explored with the same amount of program executions. However, creating a down-sample randomly might exclude important cases from the current down-sample for a number of generations, while cases that measure the same behavior (synonymous cases) may be overused despite their redundancy. In this work, we introduce Informed Down-Sampled Lexicase Selection. This method leverages population statistics to build down-samples that contain more distinct and therefore informative training cases. Through an empirical investigation across two different GP systems (PushGP and Grammar-Guided GP), we find that informed down-sampling significantly outperforms random down-sampling on a set of contemporary program synthesis benchmark problems. Through an analysis of the created down-samples, we find that important training cases are included in the down-sample consistently across independent evolutionary runs and systems. We hypothesize that this improvement can be attributed to the ability of Informed Down-Sampled Lexicase Selection to maintain more specialist individuals over the course of evolution, while also benefiting from reduced per-evaluation costs.

==> 2023-09-12-results.tex <==
\section{Results and Discussion}\label{sec:Results}
We discuss the success rates achieved by both GP systems using standard lexicase selection, random down-sampling, and different IDS configurations. Further, we study how the composition of the down-samples found by IDS changes over the number of generations. 


\subsection{Informed Down-Sampling Improves Problem-solving Success} 

Tables~\ref{tab:push_results} and~\ref{tab:ge_results} show the success rates for PushGP and G3P respectively on the chosen program synthesis benchmark problems for different parameter configurations. 
We define success rate as the number of runs that result in a program that passes the complete training set, as well as the entire unseen test set. 


For random down-sampling and IDS, we measured solutions on only the down-samples during the actual run.  As such, we execute these runs to the maximum generational limit and then conduct a post hoc analysis to see if any solutions passed all of the training cases.
If so, this is the solution that we then evaluate on the unseen test set to determine whether it generalizes or not.

For all configurations studied, we report success rates based on 100 runs. For each benchmark problem, we highlight in \textbf{bold} the best success rate at each of the down-sample sizes. Problem names in \textbf{bold} are those where an informed down-sampling run outperformed random at \emph{both} down-sample rates on that problem. Problem names that are \underline{underlined} are those where a random down-sampling run outperformed an informed down-sampling run at both down-sample rates.
Asterisks signify results that are significantly better than random down-sampling \emph{at the same down-sample size}. Standard lexicase selection was not included in our statistical analyses, as IDS is presented to improve upon random down-sampling at a fixed down-sample size. We performed significance analysis with a two proportion z-test and Bonferroni-Holm correction. Shown with * are those significant at the $\alpha=0.1$ level, ** the $\alpha=0.05$ level, and *** the $\alpha=0.01$ level.


\renewcommand{\arraystretch}{1.35}
\definecolor{lightgray}{gray}{0.9}
%\newcommand{\sig}[1]{\textbf{\underline{#1}}}
\newcommand{\sig}[1]{\textbf{#1}}

\afterpage{
\begin{landscape}
\begin{table}[h!]
\centering
\vspace*{30mm}
\caption{Number of generalizing solutions (successes) out of 100 runs achieved by PushGP on the test set.
} 
%\vspace{0.11cm}}
\label{tab:push_results}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|c|ccccc|ccccc}
\hline
  \multicolumn{1}{l|}{\textbf{Method}} & \textbf{Lex} &  \textbf{Rnd}&  \multicolumn{4}{c|}{\textbf{IDS}}&  \textbf{Rnd} & \multicolumn{4}{c}{\textbf{IDS}} \\
  \multicolumn{1}{l|}{\textbf{ $r$ }} & \textbf{-} &   \multicolumn{5}{c|}{\textbf{0.05}} & \multicolumn{5}{c}{\textbf{0.1}} \\
  \multicolumn{1}{l|}{\textbf{$\rho$}} & \textbf{-} &  \textbf{-}& \textbf{1} & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & \textbf{-}& \textbf{1} & \textbf{0.01} & \textbf{0.01} & \textbf{0.01}  \\
  \multicolumn{1}{l|}{\textbf{$k$}} & \textbf{-} &  \textbf{-}& \textbf{1} & \textbf{1} & \textbf{10} & \textbf{100} & \textbf{-}& \textbf{1} & \textbf{1} & \textbf{10} & \textbf{100}  \\
\hline
\hline

 \sig{Count Odds} &     24 &    25 &    43*** &    99*** &    \sig{100***} &    98*** &    26 &   55*** &    95*** &    \sig{99***} &    97***  \\ 


\rowcolor{lightgray}
 \textbf{Find Pair} &    5 &    27 &    9 &    32 &    32 &    \textbf{36} &    15 &    7 &    19 &    19 &    \textbf{21}    \\ 


\sig{Fizz Buzz} &    13 &    64 &    2 &    85*** &   94*** &    \sig{95***} &    45 &    3 &    75 &    78* &    \sig{81**}    \\ 

\rowcolor{lightgray}
\sig{Fuel Cost} &     41 &    72 &    1 &    83 &   \textbf{85} &    83 &    \textbf{76} &    7 &    69 &    72 &    70    \\ 

 \sig{GCD}  &     20 &    74 &    4 &    \textbf{76} &    67 &    69 &    54 &    6 &    56 &    \textbf{63} &    62    \\ 


\rowcolor{lightgray}
 Grade &    0 &    0 &    0 &    0 & \sig{1} &    0 &    \sig{1} &    0 &  0 &    \sig{1} &    \sig{1}    \\ 


 \sig{Scrabble Score} &    8 &    8 &    6 &    69*** &    64*** &    \sig{75***} &    16 &    9 &    55*** &    \textbf{74***} &    64***    \\ 

 
\rowcolor{lightgray}

\underline{\smash{Small or Large}} &     34 &    \textbf{93} &    37 &    69 &    69 &    69 &    \textbf{69} &    39 &    60 &    66 &    54   \\ 
\hline
\end{tabular}
\end{table}
\end{landscape}
}



\afterpage{
\begin{landscape}
\begin{table}[h!]
\centering
\vspace*{30mm}
\caption{Number of generalizing solutions (successes) out of 100 runs achieved by G3P on the test set. 
}\label{tab:ge_results}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|c|ccccc|ccccc}
\hline
  \multicolumn{1}{l|}{\textbf{Method}} & \textbf{Lex} &  \textbf{Rnd}&  \multicolumn{4}{c|}{\textbf{IDS}}&  \textbf{Rnd} & \multicolumn{4}{c}{\textbf{IDS}} \\
  \multicolumn{1}{l|}{\textbf{$r$ }} & \textbf{-} &   \multicolumn{5}{c|}{\textbf{0.05}} & \multicolumn{5}{c}{\textbf{0.1}} \\
  \multicolumn{1}{l|}{\textbf{$\rho$}} & \textbf{-} &  \textbf{-}& \textbf{1} & \textbf{0.01} & \textbf{0.01} & \textbf{0.01} & \textbf{-}& \textbf{1} & \textbf{0.01} & \textbf{0.01} & \textbf{0.01}  \\
  \multicolumn{1}{l|}{\textbf{$k$}} & \textbf{-} &  \textbf{-}& \textbf{1} & \textbf{1} & \textbf{10} & \textbf{100} & \textbf{-}& \textbf{1} & \textbf{1} & \textbf{10} & \textbf{100}  \\
\hline
\hline


Count Odds &    65 &    \textbf{66} &    45 &    53 &    62 &    63 &    67 &    58 &    60 &    58 &    \textbf{72}    \\ 

\rowcolor{lightgray}
 Find Pair &    0 & 0 & 0 & \textbf{1} & 0 & 0 & \textbf{1} & 0 & 0 & \textbf{1} & 0     \\ 

 \textbf{Fizz Buzz}&   62 &    83 &    50 &    84 &    78 &    \textbf{85} &    78 &    53 &    81 &    \textbf{89} &    72    \\ 

 \rowcolor{lightgray}
 Fuel Cost&    33 &    \textbf{34} &    17 &    28 &    27 &    29 &    29 &    21 &    21 &    25 &    \textbf{33}    \\ 
 
 GCD  & 0 & \textbf{1} & 0 & 0 & 0 & \textbf{1} & 0 & 0 & 0 & 0 & 0    \\ 


\rowcolor{lightgray}

 \textbf{Grade} &    36 &    39 &    29 &    51 &    \textbf{57*} &    44 &    44 &    37 &    46 &    \textbf{51} &    48    \\ 

 
 Scrabble Score &    6 & 10 & 1 & \textbf{11} & 10 & 10 & \textbf{14} & 0 & 6& 3 & 3  \\ 

 
\rowcolor{lightgray}
 \textbf{Small or Large}  &    41 &    52 &    49 &    54 &    \textbf{63} &    \textbf{63} &    59 &    52 &    57 &    55 &    \textbf{63}    \\ 




 
\hline
\end{tabular}
\end{table}
\end{landscape}
}

% regex for lexicase without the word seleciton after: lexicase[\s](?!selection)


For the PushGP results, let us consider the \emph{Fizz Buzz} problem. Standard lexicase selection had 13 successful runs. Using random down-sampling at the $0.05$ down-sampling rate improved this result to 64, in line with the findings of \cite{Helmuth2021benefits}. Using the same down-sampling rate with IDS, a $0.01$ parent rate, and $k=100$ yielded $95$ successful runs. This is significantly better than random down-sampling at the $0.01$ level. This is an important result as IDS is significantly improving on random down-sampling, which in turn improves on lexicase selection. Another set of PushGP IDS runs where we observed significant improvements were those of the \emph{Count Odds} problem. While standard lexicase selection achieves 24 successes, random down-sampling at either down-sample rate ($r=0.05$ or $r=0.1$) does not produce more than 26 successful runs. The failure to meaningfully improve success rates by random down-sampling seemed to be addressed by informed down-sampling. 
This is clear as informed down-sampling at all configurations ensures that close to if-not-all 100 runs successfully generalize to the held out test set. This and similar results hint that while randomly down-sampled lexicase selection works well usually, there are some problems where important cases might be being dropped out, resulting in a similar performance to standard lexicase selection 
despite the increased search generations. Informed down-sampling has the ability to improve success rates both when random down-sampling improves upon standard lexicase selection, and when it does not.

Only one configuration of G3P resulted in a significant improvement on random down-sampling at the same down-sample rate. For the Grade problem at the $0.05$ down-sample rate, we see significantly more successes when using IDS with $\rho = 0.01$ and $k = 10$. For this problem, using this informed down-sample configuration resulted in 57\% of the runs yielding a generalizing solution, where, using random down-sampling resulted in only 39\% of the runs yielding a success.
The fact that only a single configuration of IDS resulted in a significant improvement suggests that the problem-solving benefits of using IDS are representation- and problem-dependent, motivating future work to continue improving IDS to achieve more universal improvements to problem-solving success. 

We have a number of hypotheses explaining this improved performance. The first of these is that the informed down-sampling procedure increases the number of specialists (individuals exceptional on a few cases, but have a high \emph{total} error) that survive over the course of evolutionary time. These individuals could be better maintained with IDS as the cases they are exceptional on are still placed in the down-samples throughout evolution, preventing them from being lost as could happen when randomly down-sampling.

Another hypothesis for IDS's improved performance is that it reduces the computation used to evaluate individuals on synonymous cases.
When two cases are fully synonymous, all individuals that solve one case solve the other as well. When using lexicase selection, having both of these cases in the down-sample would result in little difference in the probability of selecting each individual compared to having only one case in the down-sample. After one of the two cases has been used to filter the pool of candidate solutions, the other will have no filtering pressure because all remaining individuals perform identically on the synonymous cases. Having a synonymous case \textit{does} increase the chance that one of the two cases appears earlier in the shuffled case ordering, producing a minor (though perhaps undesired) change in selection probability. Synonymous (or near synonymous) cases additionally take spots in the down-sample that cannot be allocated to other, more-informative cases. When using IDS, we ensure that the first few cases added to the down-sample measure relatively different behaviors. This may allow IDS to select a larger variety of individuals than random down-sampling, instead approximating the variety that could be selected by full lexicase selection.

These results, in general, make it clear that informed down-sampling by farthest first traversal is significantly outperforming randomly down-sampled lexicase selection on a portion of these program synthesis benchmark problems for the PushGP evolutionary framework. The G3P results are less clearly in favor of informed down-sampling, but still point to minor improvements in success rates.
It is important to note that all of our down-sampled runs (besides full-information) consistently and significantly outperform standard lexicase selection, which has in turn been shown to significantly outperform other selection strategies. This result agrees with that of \cite{helmuth_benchmarking_2020}, showing down-sampled lexicase selection being, before this work, the state of the art in program synthesis with genetic programming. Our informed down-sampling runs outperform random down-sampling (higher success rate for both down-sample rates) on 6/8 of the problems we studied for PushGP, with 3/8 of them being statistically significant. For G3P, informed down-sampling improves on 3/8 problems, with 1/8 being significant. 

Random down-sampling outperformed informed down-sampling (across both down-sampling levels) on only one problem (\emph{Small or Large}) for PushGP, and none for G3P. For \emph{Small or Large} with PushGP, we see that the worse performance with informed down-sampling can be attributed to a lower generalization rate (and not worse performance on the training sets). The generalization rates can be found in Appendix Table~\ref{tab:push_generalization} for PushGP and Appendix Table~\ref{tab:ge_generalization} for G3P. Future work should explore the effect that informed down-sampling has on generalization in more depth.

Appendix~\ref{appendix:sizes} shows the distributions of program size across the runs that were performed for this work. Despite the larger generational limit, there does not appear to be any significant bloating that occurs during our down-sampled runs when compared to our lexicase selection runs, despite the 10x-20x larger generational limit. This provides evidence that the method we used to ensure that all programs use similar computational resources is valid, as there are not drastic differences in program size (and thus evaluation cost). Furthermore, we employ strict evaluation limits for our PushGP runs, where programs are cut off after they reach the step limit of 200 steps. For G3P, we have a strict looping limit of 1000 iterations.

Although we introduce a variety of hyperparameters in this work, we found the most consistent improvement yielded by choosing $r=0.05, \rho=0.01, k=10$. As such, we recommend these hyperparameters as a starting point for future investigation.

\subsection{Using Smaller Informed Down-Samples Tends to Improve Success Rates}

In general, our IDS runs at a 0.05 down-sample rate have a higher success rate than their equivalent counterparts at the 0.1 down-sample rate. This difference is likely due to the fact that the runs at a 0.1 down-sample rate have a substantially lower generational limit, meaning that we are exploring a smaller portion of the space of possible solution programs. With 200 training cases, our down-sample contains 10 and 20 cases respectively for the 0.05 and 0.1 down-sample rates. A possible reason for the improved performance at 0.05 is that a larger proportion of these cases are indeed our distinct, or informative, cases. Note that once the Farthest First Traversal process selects a representative case for every synonymous group in the down-sample, every remaining solution's minimum distances to the current sample will be equal to 0, so the selections are performed randomly to fill the rest of the cases. Since we are using the same problems, with the same number of behavioral niches, we will see the runs with 20 cases in the down-sample having more synonymous cases in the down-sample. Due to the fact that the content of the training cases is not notably more informative to make up for the decreased generational limit, we see a lower success rate. We will analyze the specific cases that compose the down-samples in section~\ref{sec:caseComp}.

The exceptions to this trend are the full information down-sampling runs. For these runs, the larger down-samples tend to perform better. This result is likely due to the fact that the generational limit was set to 300 for both sampling levels (as they both evaluate all individuals on all test cases), and so having a smaller down-sample size would not change the number of evaluations. With more cases in the sample, the GP method can take into account more information when performing selection, which could result in more informed search. The magnitude of the differences for success rate across sample size for the full IDS runs suggests that there are diminishing returns for including more cases in the sample.


\subsection{Informed Down-Sampling Automatically Discovers Important Training Cases}\label{sec:caseComp}

To gain a deeper insight into how IDS composes down-samples, we visualize how the selected training cases (used for a down-sample) develop over the generations of an evolutionary run.



Figures~\ref{fig:push_downsample_comp_1} and~\ref{fig:ggg_downsample_comp_1} show the composition of down-samples for every problem at every generation using PushGP (Fig.~\ref{fig:push_downsample_comp_1}) and G3P (Fig.~\ref{fig:ggg_downsample_comp_1}) with down-sample rate $r=0.05$. We present results for a full information configuration ($\rho=1$ and $k=1$) as well as a sparse information configuration ($\rho=0.01$ and $k=10$). We chose to analyze both a full information and sparse information run in order to see whether our sparse information configurations are finding the same training cases to be informative as if we had used all parents to evaluate the distances between training cases.

The plots show how often certain training cases are included in the down-sample at every generation, averaged over all active runs. Each row represents a case in the training data, ordered by its position in the training set. The training sets used were generated by first adding some human-expert defined edge cases, and filling the rest with cases that were randomly generated by an function that already implements our desired program (oracle function). For each figure, there is a single marker on the $y$-axis that shows where exactly the expert-case cutoff for the training set was. Thus, the rows above the marker in the visuals are representing cases that humans determined to be important based on the problem definition. 

Brighter colors imply that a case is included more often, darker colors imply a lower number of inclusions.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.85\textwidth]{4x2_Push_1.pdf}
    \caption{Down-sample composition over generations for PushGP with 0.05 down-sample rate for a full information ($\rho=1$ and $k=1$) and a sparse information configuration ($\rho=0.01$ and $k=10$). }
    \label{fig:push_downsample_comp_1}
\end{figure}

\begin{figure}[!ht]
\ContinuedFloat
    \centering
    \includegraphics[width=0.85\textwidth]{4x2_Push_2.pdf}
    \caption{Continued.}
    \label{fig:push_downsample_comp_2}
\end{figure}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.85\textwidth]{4x2_G3P_1.pdf}
    \caption{Down-sample composition over generations for G3P with 0.05 down-sample rate for a full information ($\rho=1$ and $k=1$) and a sparse information configuration ($\rho=0.01$ and $k=10$). \\ }
    \label{fig:ggg_downsample_comp_1}
\end{figure}

\begin{figure}[!ht]
\ContinuedFloat
    \centering
    \includegraphics[width=0.85\textwidth]{4x2_G3P_2.pdf}
    \caption{Continued.}
    \label{fig:ggg_downsample_comp_2}
\end{figure}


For PushGP (Figure~\ref{fig:push_downsample_comp_1}), we see that the configurations with sparse information often include the same cases in the down-sample as the runs with full information. This result means that by using a parent sampling rate of $\rho = 0.01$ and a case distance evaluation schedule parameter of $k=10$, we can significantly reduce the number of evaluations needed to calculate distances between cases, while still maintaining a good approximation to the ground truth (full information, where we use all parents every generation to calculate distances). However, the composition for our sparse information runs are slightly more noisy than that for full information, suggesting that using parent sampling could introduce some extra stochasticity to the down-sample creation process.

For all studied benchmark problems, we see that IDS has a strong bias toward specific training cases that are included substantially more often in the down-sample. 
These selected training cases are mainly consistent with the human-defined edge cases that exist at the beginning of the training set. This result shows that informed down-sampling is indeed often finding the same cases to be informative as those that a human expert would, without any knowledge of the problem definition.
However, with IDS, we can draw further comparisons of informativeness within this expert-defined groups of cases. This can be seen as some cases are selected more often that others \emph{within} the first several cases.


We then look at the labels of the specific training cases that are found to be important. We see that these training cases make sense to be included more often than others in the down-samples. Note that the labels of the specific training cases are not included in the plots for simplicity, but can be queried based on their specific index in the data sets provided in our code implementation.

For example, for the \emph{Small or Large} problem, cases around the decision boundaries as well as numbers between $0$ and $1000$ are more often included. 
For the \emph{Grade} problem, those edge cases with very close decision boundaries are included while the ones with far away boundaries are not taken into account for the down-sample.
For \emph{Fuel Cost}, nearly all of the human defined edge cases are found to be important, while for the \emph{GCD} problem the first two cases in particular make it in nearly every down-sample, while the rest are selected less often.

For the \emph{Scrabble Score} problem, we see that the first edge cases, which specify the score for each letter, does not seem to be informative at all. This result is not surprising, as this information is already available to PushGP through a vector with these scores on the vector stack. However, the three edge cases after them with empty strings and special characters as input are included a lot.
For \emph{Count Odds}, the edge cases denoting empty lists, or lists with zero or a single odd number were found to be important, indicating that those contain all the important information to learn what are odd and even numbers as well as how to handle a list.
For \emph{Fizz Buzz}, all edge cases seem important while for the \emph{Find Pair} problem only those edge cases with lists of length $3$ are consistently included. Those lists of length $2$ in the edge cases are represented in the down-sample less often.

Lastly, we see that the composition of the down-sample stays rather stable during the evolutionary run for the PushGP system, explaining why there is only a small difference in our experiments between calculating the distances every $k=1$ and $k=100$ generations (see Table~\ref{tab:push_results}).



For G3P (Fig~\ref{fig:ggg_downsample_comp_1}), we see similar results as with PushGP. However, for the problems that require iterative structures to be solved (\emph{Count Odds}, \emph{Find Pair}) we see that the down-sample quickly dissolves into random noise instead of any form of structure. This dynamic occurs despite the fact that the same edge cases as with PushGP are initially identified in the first few generations. This result is not surprising as finding iterative structures is known to be challenging for grammar-guided approaches, as such structures are difficult to be built step-by-step guided by the performance on a set of training cases. \citep{sobania2020challenges, sobania2022comprehensive}. Another difference between the case compositions are that, while IDS with G3P tends to discover the same cases as those found with PushGP, their use is less consistent, resulting in lines that are more faint than those for PushGP. Both of these hypotheses could help explain the relatively worse improvement that IDS yields for G3P than for PushGP.

However, for the problems that require conditionals, like \emph{Small or Large} and \emph{Grade}, we see that the important cases are identified and used during evolution. This result is also reflected in the success rates compared to random down-sampling (see Table~\ref{tab:ge_results}).

Interestingly, IDS identifies many of the same cases as important for G3P as well as PushGP. This result suggests that the structure of the problem itself determines which cases are important rather than the considered representation. This dynamic makes IDS potentially useful across many different systems and approaches. 

Across both systems, we see that the important cases are determined and selected very early in evolution, despite the relatively uninformative environment at the beginning of evolution. At the beginning of the run, most cases are failed by all individuals, making it hard to distinguish between informative and uninformative cases. An option that could help address this issue would be to use raw fitness values to measure the distance between test cases. However, using this system would require the definition of a similarity function based on fitness values, which could introduce hyper-parameters that detract from the simplicity of our approach.


